Parameter-Efficient Cross-lingual Transfer of Vision and Language Models via Translation-based Alignment

Pre-trained vision and language models such as CLIP have witnessed remarkable success in connecting images and texts with a primary focus on English texts. Despite recent efforts to extend CLIP to support other languages, disparities in performance among different languages have been observed due to uneven resource availability. Additionally, current cross-lingual transfer methods of those pre-trained models would consume excessive resources for a large number of languages. Therefore, we propose a new parameter-efficient cross-lingual transfer learning framework that utilizes a translation-based alignment method to mitigate multilingual disparities and explores parameter-efficient fine-tuning methods for parameter-efficient cross-lingual transfer. Extensive experiments on XTD and Multi30K datasets, covering 11 languages under zero-shot, few-shot, and full-dataset learning scenarios, show that our framework significantly reduces the multilingual disparities among languages and improves cross-lingual transfer results, especially in low-resource scenarios, while only keeping and fine-tuning an extremely small number of parameters compared to the full model (e.g., Our framework only requires 0.16\% additional parameters of a full-model for each language in the few-shot learning scenario). The codes are available at \url{https://github.com/eric-ai-lab/PECTVLM}. The codes are available at \url{https://github.com/eric-ai-lab/PECTVLM}.

==> 0_method_old.tex <==
\section{Method old}



\subsection{Different scenarios}
\subsubsection{Parameter Efficiency}

\subsubsection{Machine Translation}


\subsubsection{Parallel Corpus}
Compared with non-parallel data, parallel data or sentences in different languages describing the same picture provide more information. For example, ...
In this paper, we explore how to better take advantage of parallel corpus as well as the combination of translation.

\subsubsection{Low-resourced Language}
For some low-resourced languages, there may not exists enough training data. In this scenario, transferring knowledge from other language or some zero-shot learning method(e.g., prompt) may help.


\subsection{Parameter-Efficient Tuning}
We explore several state-of-the-art pet method(prompt, LoRA, Compacter, Adapter). These methods preserve most of the performance.

We plot the trend of the effect with the number of parameters



\subsection{Translation Guidance}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/translationguidance.png} 
    \caption{Translation Guidance\jialu{TODO}{Plot this figure with softwares}}
    \label{fig:translation_guidance}
\end{figure}

We add text-text loss(MSE) between language features, as shown by the three red dashed lines in Figure~\ref{fig:translation_guidance}. Intuitively, the distance of 3 \& 2 hould be less than 1 and the performance of 3 may be the best because it is in English.
\subsection{Abundant other language data + few-shot target language data}
Firstly we train the model on English dataset. From Table \ref{fig:translation_guidance}, we can observe that performance of all languages are improved. When we continue to train the model on target language on this basis, performance continue to be improved. The improvement is very significant compared with directly training on target language dataset without using English dataset.

\subsection{Prompt for Zero-Shot}
Explore these method: 
1. add prompt in corresponding language to texts.
2. Simply add prompt in English to text. 
3. translate the sentences to English then add prompt in English
We found 3 with prompt "A photo of" works best.


==> 0_results.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{table*}[th]

  	\resizebox{2.0\columnwidth}{!}{
\begin{tabular}{lcclccccccccccccc}
\hline
\multicolumn{1}{l|}{}     & \multicolumn{3}{c|}{Components}             & \multicolumn{13}{c}{XTD}                                                        \\ \cline{2-17} 
\multicolumn{1}{l|}{}     & MT & PCG & \multicolumn{1}{l|}{PET/FT}         & en    & de    & fr    & es    & it    & ko    & pl    & ru    & tr    & zh    & \multicolumn{1}{l|}{jp}    & avg   & avg$_\text{-en}$ \\ \hline
\multicolumn{17}{c}{Zero-Shot}                                                                     \\ \hline
\multicolumn{1}{l|}{(0)*}  & \checkmark  &     & \multicolumn{1}{l|}{}            & 62.06 &	60.56 &	60.56 & 	59.72 &	58.78 &	58.00 &	60.11 &	53.72 &	60.06 &	56.72 &	\multicolumn{1}{l|}{50.72} &	58.27 &	57.90 \\
\multicolumn{1}{l|}{(1)}  &    &     & \multicolumn{1}{l|}{}            & 63.44 & 59.94 & 60.06 & 58.90 & 60.72 & 51.00 & 61.50 & 56.11 & 59.28 & 59.28 & \multicolumn{1}{l|}{47.44} & 57.97 & 57.42    \\
\multicolumn{1}{l|}{(2)}  & \checkmark  &     & \multicolumn{1}{l|}{}            & 63.44 & 61.11 & 61.33 & 62.33 & 61.17 & 61.44 & 61.50 & 54.83 & 61.67 & 58.00 & \multicolumn{1}{l|}{52.72} & 59.96 & 59.61    \\
\multicolumn{1}{l|}{(3)}  &    &     & \multicolumn{1}{l|}{$\text{prompt}_\text{tgt}$} & 64.06 & 60.83 & 60.33 & 62.06 & 61.22 & 49.00 & 61.00 & 56.00 & 59.39 & 59.33 & \multicolumn{1}{l|}{48.06} & 58.30 & 57.72    \\
\multicolumn{1}{l|}{(4)}  &    &     & \multicolumn{1}{l|}{prompt}      & 64.06 & 60.72 & 59.89 & 61.78 & 61.28 & 51.67 & 62.06 & 56.00 & 60.11 & 59.78 & \multicolumn{1}{l|}{47.83} & 58.65 & 58.11    \\
\multicolumn{1}{l|}{(5)}  & \checkmark  &     & \multicolumn{1}{l|}{prompt}      & 63.94 & 61.17 & 62.00 & 62.17 & 61.56 & 60.50 & 62.44 & 55.44 & 61.83 & 58.67 & \multicolumn{1}{l|}{53.33} & 60.28 & 59.91    \\ \hline
\multicolumn{17}{c}{Few-Shot}                                                                                                                                                                           \\ \hline
\multicolumn{1}{l|}{(6)}  &    &     & \multicolumn{1}{l|}{Compacter}   & 63.67 & 60.61 & 60.44 & 60.50 & 61.33 & 52.06 & 62.67 & 55.94 & 59.72 & 59.39 & \multicolumn{1}{l|}{49.00} & 58.67 & 58.17    \\
\multicolumn{1}{l|}{(7)}  &    &     & \multicolumn{1}{l|}{Adapter}     & 64.44 & 61.17 & 60.61 & 60.72 & 61.39 & 52.17 & 62.83 & 56.44 & 59.50 & 59.67 & \multicolumn{1}{l|}{49.17} & 58.92 & 58.37    \\
\multicolumn{1}{l|}{(8)}  &    &     & \multicolumn{1}{l|}{LoRA}        & 64.50 & 61.10 & 60.39 & 60.89 & 61.67 & 53.06 & 61.94 & 56.67 & 60.50 & 59.82 & \multicolumn{1}{l|}{49.56} & 59.10 & 58.56    \\
\multicolumn{1}{l|}{(9)}  &    &     & \multicolumn{1}{l|}{FT}          & 64.67 & 61.83 & 60.67 & 61.33 & 62.00 & 52.22 & 62.61 & 56.33 & 60.39 & 59.72 & \multicolumn{1}{l|}{48.61} & 59.13 & 58.57    \\
\hline
\multicolumn{1}{l|}{(10)} & \checkmark  &     & \multicolumn{1}{l|}{prompt(3)}   & 63.94 & 61.17 & 62.00 & 62.17 & 61.56 & 60.50 & 62.44 & 55.44 & 61.83 & 58.72 & \multicolumn{1}{l|}{53.33} & 60.28 & 59.92    \\
\multicolumn{1}{l|}{(11)} & \checkmark  &     & \multicolumn{1}{l|}{prompt(20)}  & 62.72 & 59.89 & 60.50 & 60.28 & 59.83 & 59.44 & 60.22 & 54.33 & 60.00 & 58.11 & \multicolumn{1}{l|}{53.11} & 58.95 & 58.57    \\
\multicolumn{1}{l|}{(12)} & \checkmark  &     & \multicolumn{1}{l|}{Compacter}   & 63.67 & 61.22 & 61.28 & 61.50 & 61.11 & 61.44 & 62.00 & 55.50 & 62.22 & 58.39 & \multicolumn{1}{l|}{53.72} & 60.19 & 59.84    \\
\multicolumn{1}{l|}{(13)} & \checkmark  &     & \multicolumn{1}{l|}{Adapter}     & 64.44 & 61.72 & 61.89 & 61.56 & 61.11 & 61.00 & 63.06 & 55.44 & 62.11 & 58.56 & \multicolumn{1}{l|}{54.00} & 60.44 & 60.05    \\
\multicolumn{1}{l|}{(14)} & \checkmark  &     & \multicolumn{1}{l|}{LoRA}        & 64.50 & 62.00 & 61.89 & 61.72 & 61.17 & 61.33 & 62.17 & 55.56 & 62.39 & 58.89 & \multicolumn{1}{l|}{54.11} & 60.52 & 60.12    \\
\multicolumn{1}{l|}{(15)} & \checkmark  &     & \multicolumn{1}{l|}{FT}          & 64.67 & 61.89 & 62.00 & 62.17 & 61.44 & 61.00 & 63.00 & 56.11 & 62.00 & 59.50 & \multicolumn{1}{l|}{53.83} & 60.69 & 60.29    \\
\hline
\multicolumn{1}{l|}{(16)} & \checkmark  & \checkmark   & \multicolumn{1}{l|}{Adapter}     & 64.44 & 61.89 & 61.83 & 61.89 & 61.83 & 61.56 & 62.78 & 55.83 & 62.11 & 59.06 & \multicolumn{1}{l|}{54.17} & \textbf{60.67} & \textbf{60.30}    \\
\multicolumn{1}{l|}{(17)} & \checkmark  & \checkmark   & \multicolumn{1}{l|}{LoRA}        & 64.50 & 61.94 & 62.00 & 62.00 & 61.83 & 61.65 & 62.72 & 55.94 & 62.33 & 59.84 & \multicolumn{1}{l|}{54.22} & \textbf{60.82} & \textbf{60.45}    \\
\multicolumn{1}{l|}{(18)} & \checkmark  & \checkmark   & \multicolumn{1}{l|}{FT}          & 64.67 & 62.17 & 62.22 & 61.94 & 61.89 & 61.56 & 63.11 & 56.06 & 62.28 & 59.83 & \multicolumn{1}{l|}{54.17} & \textbf{60.90} & \textbf{60.52}    \\ \hline
\end{tabular}
}
\caption{Results on XTD dataset in zero-shot and few-shot learning senario. We bold the best score for different tuning approach respectively. "avg$_\text{-en}$" represents average score without English. "*" represents we use original monolingual text encoder of CLIP and translate all the text inputs into English.The number in parentheses after "prompt" represents the number of tokens.}
\label{table:XTD}
\end{table*}

\begin{table}[t]
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcclcccccc}
\hline
\multicolumn{1}{l|}{}     & \multicolumn{3}{c|}{Components}        & \multicolumn{6}{c}{Multi30K}                                                                                    \\ \hline
\multicolumn{1}{l|}{}     & MT & PCG & \multicolumn{1}{l|}{PET/FT}    & en    & cs             & de             & \multicolumn{1}{c|}{fr}             & avg            & avg$_\text{-en}$       \\ \hline
\multicolumn{10}{c}{Zero-Shot}                                                                                                                                                       \\ \hline
\multicolumn{1}{l|}{(0)*}  &  \checkmark  &     & \multicolumn{1}{l|}{}       & 66.50 & 63.25          & 66.05          & \multicolumn{1}{c|}{66.70}          & 65.63          & 65.33          \\
\multicolumn{1}{l|}{(1)}  &    &     & \multicolumn{1}{l|}{}       & 66.65 & 64.50          & 65.00          & \multicolumn{1}{c|}{65.60}          & 65.44          & 65.03          \\
\multicolumn{1}{l|}{(2)}  & \checkmark  &     & \multicolumn{1}{l|}{}       & 66.65 & 65.25          & 66.00          & \multicolumn{1}{c|}{66.15}          & 66.01          & 65.80          \\
\multicolumn{1}{l|}{(5)}  & \checkmark  &     & \multicolumn{1}{l|}{prompt} & 67.80 & 66.60          & 66.50          & \multicolumn{1}{c|}{67.10}          & 67.00          & 66.73          \\ \hline
\multicolumn{10}{c}{Full-Dataset}                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{(8)}  &    &     & \multicolumn{1}{l|}{LoRA}   & 75.20 & 72.55          & 73.70          & \multicolumn{1}{c|}{75.30}          & 74.19          & 73.85          \\
\multicolumn{1}{l|}{(9)}  &    &     & \multicolumn{1}{l|}{FT}     & 76.10 & 74.55          & 74.80          & \multicolumn{1}{c|}{75.45}          & 75.23          & 74.93          \\
\hline
\multicolumn{1}{l|}{(14)} & \checkmark  &     & \multicolumn{1}{l|}{LoRA}   & 75.35 & 73.65          & 73.30          & \multicolumn{1}{c|}{75.95}          & 74.56          & 74.30          \\
\multicolumn{1}{l|}{(15)} & \checkmark  &     & \multicolumn{1}{l|}{FT}     & 76.10 & 75.25          & 74.65          & \multicolumn{1}{c|}{76.00}          & 75.50          & 75.30          \\
\hline
\multicolumn{1}{l|}{(17)} & \checkmark  & \checkmark   & \multicolumn{1}{l|}{LoRA}   & 75.35 & \textbf{73.90}          & \textbf{73.75}          & \multicolumn{1}{c|}{\textbf{76.50}}          & \textbf{74.88}          & \textbf{74.72}          \\
\multicolumn{1}{l|}{(18)} & \checkmark  & \checkmark   & \multicolumn{1}{l|}{FT}     & 76.10 & \textbf{75.85} & \textbf{75.05} & \multicolumn{1}{c|}{\textbf{76.70}} & \textbf{75.93} & \textbf{75.87} \\ \hline
\end{tabular}
}
\caption{Results on Multi30K dataset in zero-shot and few-shot learning senario. We bold the best score for different tuning approach respectively. "avg$_\text{-en}$" represents average score without English. "*" represents we use original monolingual text encoder of CLIP and translate all the text inputs into English.}
\label{table:multi30k}
\end{table}

% We demonstrate the different results produced by different components in the unified structure in Table~\ref{table:XTD} and Table~\ref{table:multi30k}. Results are compared in both zero-shot and few-shot settings on XTD. We number the rows in tables with the same number if the combination is the same. For a more obvious comparison, we report Recall@1 score in all experiments. 
\subsection{The Unified Framework}

% \paragraph{Machine Translation.}
% Compared with keeping the text input in the target language embedding space, translating texts into pivot language significantly improves the performance on average(6 vs 12; 7 vs 13; 8 vs 14; 9 vs 15). Machine translation has demonstrated its power in most languages except Chinese and Russian on XTD dataset. Results of MT indicate that mapping all languages to pivot language embedding space is a feasible and effective way to address the multilingual disparity. Meanwhile, since MT maps all languages into the same language embedding space, it is much easier to align texts with the same meaning but translated from different languages, laying the foundation for the PCG method.



\paragraph{Parallel Corpus Guidance.}
% We show the results of different routines mentioned in Section~\ref{sec:PCG} in Table~\ref{table:ablation} (A, B, E). As seen, MSE loss in pivot language embedding space (E) performs the best. This may be because Multilingual-CLIP uses MSE loss in the pre-training stage, and loss between text-text pair provides stronger constraints than text-image pair to the target language.
% We have demonstrated the importance of MT, and that is the reason why we guide the text embedding in the same language space. From the results in Table~\ref{table:XTD} and Table~\ref{table:multi30k}, PCG method further improves the average performance of the Multilingual-CLIP approximately by 0.3 on the XTD dataset and by 0.6 on the Multi30K dataset in the target language. With the help of PCG, the distribution of translated text embeddings can be guided toward true pivot language distribution.





% \paragraph{Prompt} We analyse the three combinations of prompt tuning mentioned in Section~\ref{sec:prompt_zeroshot}. It can be found that the zero-shot performance increases by simply adding prompt in English, with both text input in target language(1 vs 4) and translated into English (2 vs 5). We compare different hard prompts and find "a photo of" performs best. Other Results of other hard prompts can be found in Table~\ref{table:hard_prompt_comparation}. However, Translating English prompt into target language makes the performance decrease slightly (3 vs 4). Finally, We get the best performance by translate all the text inputs into English and adding the best English prompt to them (1 vs 5). 
% \jialu{TODO}{Analysis}

% CLIP model uses some templates like "a photo of" during the pre-training stage, so it is not unexpected that using these templates will benefit the model in zero-shot setting. With more training data, the model obtains marginal improvement or even performance decreasing by utilizing these templates. 

% \paragraph{Other PET Methods}
% We compare fine-tuning the full model with 4 popular parameter-efficient methods: Prompt, Compacter, Adapter and LoRA.

% From results shown in Table~\ref{table:XTD}, we can find that LoRA performs the best among all the PET methods, which preserves 99.9\% performance of fine-tuning (17 vs 18). We further compare LoRA and fine-tuning on Multi30K in Table~\ref{table:multi30k}. LoRA preserves 98.6\% performace of the fine-tuning while only tunes ?\% parameters. In multilingual and multitasking scenarios, PET methods are more suitable which maintain most of the effectiveness while being parameter-efficient.
% Compared with zero-shot, the performance of Prompt gets nearly no improvement with initialization from hard prompt (10). Considering the small number of parameters of hard prompt, we then use 20 random initialized tokens from a normal distribution with mean of 0 and standard deviation of 0.02 (11) but find the performance decreases.







% \subsection{Ablation}
% \subsubsection{Why Multilingual CLIP}
% Compared with original monolingual text encoder, multilingual CLIP with MT obtains better result (0 vs 2). We can found that even though the performance of monolingual CLIP on English is lower than that of multilingual CLIP, the average score  of monolingual CLIP on all languages is higher.
% Although monolingual CLIP with machine translation has shown a strong effect, it is still not as good as the multilingual CLIP, and multilingual CLIP can still process inputs in other languages when machine translation is not available.
\subsubsection{Different Guidance Methods}
\begin{table*}[h]
\resizebox{2.0\columnwidth}{!}{
\begin{tabular}{l|cll|ccccccccccc|cccc}
\hline
    &         &             &          & \multicolumn{11}{c|}{XTD}                                                                                     & \multicolumn{4}{c}{Multi30K}                          \\ \cline{5-19} 
    & Routine & Loss        & Pair     & de    & fr    & es    & it    & ko    & pl    & ru    & tr    & zh    & \multicolumn{1}{c|}{jp}    & avg\_nen & cs    & de    & \multicolumn{1}{c|}{fr}    & avg\_nen \\ \hline
A & 3    & contrastive & en-image & 62.17 & 62.00 & 62.06 & 61.78 & 61.17 & 63.11 & 56.00 & 62.33 & 59.83 & \multicolumn{1}{c|}{54.11} & 60.46    & 75.70 & 75.20 & \multicolumn{1}{c|}{76.65} & 75.85    \\
B & 3       & contrastive & en-tgt   & 61.83 & 61.94 & 61.56 & 61.50 & 60.89 & 63.11 & 55.94 & 62.39 & 59.94 & \multicolumn{1}{c|}{53.94} & 60.30    & 74.60 & 75.05 & \multicolumn{1}{c|}{76.75} & 75.47    \\
C & 1       & MSE         & en-tgt   & 62.17 & 61.06 & 61.56 & 62.28 & 52.72 & 62.78 & 57.06 & 59.94 & 59.94 & \multicolumn{1}{c|}{48.94} & 58.85    & 74.95 & 75.25 & \multicolumn{1}{c|}{76.50} & 75.57    \\
D & 2       & MSE         & en-tgt   & 62.22 & 61.11 & 61.56 & 62.11 & 52.50 & 62.78 & 56.78 & 60.06 & 60.00 & \multicolumn{1}{c|}{49.00} & 58.81    & 74.85 & 75.15 & \multicolumn{1}{c|}{76.95} & 75.65    \\
E & 3       & MSE         & en-tgt   & 62.17 & 62.22 & 61.94 & 61.89 & 61.56 & 63.11 & 56.06 & 62.28 & 59.83 & \multicolumn{1}{c|}{54.17} & \textbf{60.52}    & 75.85 & 75.30 & \multicolumn{1}{c|}{76.75} & \textbf{75.97}    \\ \hline
\end{tabular}
}
\caption{Ablation on different guidance methods.}
\label{table:ablation}
\end{table*}

% Since we have parallel data in English and target language, contrastive loss between English texts and images and contrastive between English and target language text are alternatives. We compare these two possible loss with the parallel corpus guidance in this section. As shown in the Table~\ref{table:ablation} (A, B, E), the MSE loss on en-tgt pair strategy performs best. This may be because MSE loss is use in the pre-training phase for teacher learning and loss between text embeddings provides a better supervision.

\subsubsection{Optimal $\lambda$ for Each Language}
\label{sec:ablation_lambda}
% \begin{figure*}[]
%     \centering
%     \includegraphics[width=\linewidth]{figs/ablation-lambda.png} 
%     \caption{Optimal $\lambda$ for Each Language}
%     \label{fig:ablation_lambda}
% \end{figure*}

% We plot tendancy of the result to change with $\lambda$ in Figure~\ref{fig:ablation_lambda}. In the vast majority of languages, we can see that the curve has a clear peak corresponding to the optimal $\lambda$. Most of the optimal $\lambda$s are between 0.1 and 1.



% \subsubsection{Re-training after trained on an Englihs dataset}
% \begin{table*}[h]
% \resizebox{2.0\columnwidth}{!}{
% \begin{tabular}{lll|lllllllllll|ll}
% \hline
%           &              Trained on                & Domain & en    & de    & fr    & es    & it    & ko    & pl    & ru    & tr    & zh    & jp    & Avg   & Avg_{-en} \\
%           \hline
% zeroshot  & XTD      & tgt    & 64.67 & 61.65 & 60.94 & 61.50 & 62.22 & 52.17 & 61.89 & 56.83 & 60.11 & 60.33 & 48.83 & 59.19 & 58.65    \\
% zeroshot  & XTD      & en     & 64.67 & 61.83 & 62.06 & 61.72 & 61.72 & 61.06 & 62.61 & 55.39 & 61.94 & 59.78 & 54.50 & 60.66 & 60.26    \\
% zeroshot  & Multi30k & tgt    & 67.78 & 64.17 & 65.28 & 64.61 & 65.11 & 54.39 & 66.56 & 59.94 & 65.00 & 63.56 & 51.61 & 62.55 & 62.02    \\
% zeroshot  & Multi30k & en     & 67.78 & 65.94 & 65.72 & 66.44 & 64.72 & 64.56 & 67.50 & 58.61 & 65.44 & 62.78 & 57.67 & 64.29 & 63.94    \\
% \hline
% baseline2 & train from en init(XTD)      & en     & 64.67 & 61.83 & 62.17 & 61.78 & 61.56 & 60.83 & 63.00 & 55.72 & 62.44 & 59.89 & 54.11 & 60.73 & 60.33    \\
% baseline2 & train from en init(Multi30k) & en     & 68.06 & 66.06 & 66.06 & 66.33 & 64.83 & 64.11 & 67.50 & 57.72 & 65.61 & 63.39 & 57.94 & 64.33 & 63.96  \\
% \hline
% \end{tabular}
% }
% \caption{Results on XTD. Re-train the model on other English dataset after being trained on a English dataset.}
% \label{table:retrain}
% \end{table*}
% **need to rephrase


% Table~\ref{table:fewshot} includes some results that need to be discussed. I train the model on Multi30K and XTD English dataset. Then I initialize the model with these checkpoints and train it on XTD dataset in other languages. I expected to demonstrate that training on English dataset benefits other language, an then we can continue to train it on other language datasets. But from the results, these is almost no improvement in the retraining process. I do not know why...

